Conditional Choice Probability Estimation of Dynamic Discrete Choice Models with 2-period Finite Dependence

This paper extends the work of Arcidiacono and Miller (2011, 2019) by introducing a novel characterization of finite dependence within dynamic discrete choice models, demonstrating that numerous models display 2-period finite dependence. We recast finite dependence as a problem of sequentially searching for weights and introduce a computationally efficient method for determining these weights by utilizing the Kronecker product structure embedded in state transitions. With the estimated weights, we develop a computationally attractive Conditional Choice Probability estimator with 2-period finite dependence. The computational efficacy of our proposed estimator is demonstrated through Monte Carlo simulations.

==> ReformulatingBellmanProbability.tex <==
\subsection{Reformulating Bellman equation}\label{sec:dynamic_probability_choice_problem}
For the following of this section, we omit the agent index $i$.
We reformulate the agent' dynamic decision problem as defined in \eqref{eq:bellman} in the probability space and denote his problem as the \emph{dynamic probability-choice problem}.
We show below that there is a one-to-one relationship between optimal decision rules (and value functions) in the \emph{dynamic discrete choice problem} and in the reformulated \emph{dynamic probability-choice problem} as follows.

Consider the time $t$, where prior to the realization of the state $x_t$, the agent faces a distribution of the probability of state realization $\bs \kappa_t = [\kappa_t(x): x \in \mathcal{X} ]\t$ with $\kappa_t(x) \in [0,1]$ and $\sum_{x \in \mathcal{X}} \kappa_t(x) = 1$. Instead of choosing a discrete action $d \in \mathcal{D}$ after observing a realization of the state $x$, the agent has a complete plan and chooses a decision probability over all the possible state $\mb p_t \equiv \{ p_t(d, x) : d \in \mathcal{D}/ \{ 0\}, x \in \mathcal{X} \} \in \mathcal{B}_P \subset \R^{XD}$. Note that we leave $p_t(0,x)$ out in the definition of $\mb p_t$ for each $x \in \mathcal{X}$ because the choice probabilities are subject to the constraint $p_t(d,x) \in [0,1]$ and $\sum_{d \in \mathcal{D}} p_t(d, x) = 1$.


Given an arbitrary vector of choice probabilities $\mb p_t \in \mathcal{B}_P$, 
let $\mb{u}( \mb{p}_t)$, $\mb{e}( \mb{p}_t)$ and $\mb{F}( \mb{p}_t)$ denote vectors of $\mb{p}_t$-weighted flow utility, $\mb{p}_t$-weighted expected private information and the matrix of $\mb{p}_t$-weighted transition densities:
\begin{equation}
	\mb{u}( \mb{p}_t) =  \left[\sum_{d \in \mathcal{D}}  p_t(d,1) \mathrm u(d, 1), \ldots,  \sum_{d \in \mathcal{D}}  p_t(d,X)  \mathrm u(d, X) \right]\t, 
	\label{eq:u_p}
\end{equation}  
\begin{equation} 
	\mb{e}( \mb{p}_t) =  \left[\sum_{d \in \mathcal{D}} p_t(d,1) \mb e^{\mb p_t(1)}(d, 1), \ldots,  \sum_{d \in \mathcal{D}} p_t(d,X)  e^{\mb p_t(X)}(d, X) \right]\t, 
	\label{eq:e_p}
\end{equation} 
and
\begin{equation} 
	\mb{F}( \mb{p}_t) =  \begin{bmatrix}
		\sum_{d=0}^{D}p_t(d, 1)  f( 1 | 1,  d)& \ldots & \sum_{d=0}^{D}p_t(d, x)  f( X | 1,  d) \\
		\vdots & \ddots & \vdots \\
		\sum_{d=0}^{D}p_t(d, x)  f( 1 | X,  d)& \ldots & \sum_{d=0}^{D}p_t(d, x)  f( X | X,  d) \\
	\end{bmatrix}, 
	\label{eq:F_p}
\end{equation}  
where the expected private information ${e}^{\mb p_t(x)}(d,x) $ is given by:
% of $\epsilon_t(d)$ given the choice $d$ being the optimal choice function given the value differences $\mb{\tilde v}(x)$:
\begin{equation}\label{eq:e_definition}
	{e}^{\mb p_t(x)}(d,x) = \int \epsilon_t(d)  \prod_{d'\neq d} \ind \{  \mb{\Lambda}^{-1}(d,\mb p_t(x))  + \epsilon_t(d) \ge \mb{\Lambda}^{-1}(d',\mb p_t(x)) +\epsilon_t(d') \} g(\bs{\epsilon}_t) d \bs{\epsilon}_t.
\end{equation}
with $\mb{\Lambda}^{-1}(d,\mb p_t(x))$ the $d$-th element of the $\mb{\Lambda}^{-1}(\mb p_t(x))$.
Under Assumption \ref{assumption:T1EV}, ${e}^{\mb p(x)}(d,x)  = \gamma - \ln ( p(d,x))$ for any $d\in\mathcal{D}$ as in Example \ref{example:hm_inversion}, where $\gamma \approx 0.5772156649$ is the Euler constant.

The agent faces the \emph{dynamic probability-choice problem} characterized by the utility sequence \( \big\{ \bs\kappa_t\t\big(\mb{u}( \mb{p}_t) + \mb{e}( \mb{p}_t)\big)\big\}_{t=0}^{T} \) and the deterministic transition rules $\{\bs \kappa_{t+1} = \mb{F}( \mb{p}_t)\t \bs \kappa_t \}_{t=0}^{T}$.
The decisions for the agent are a sequence of choice probabilities $\{ \mb p_t \}_{t=0}^T$ to maximize the $\mb p_t$ weighted payoffs. 
In analogue to the choice-specific value function and the expected value function, we define the probability-specific value function and the value function to the \emph{dynamic probability-choice problem} as below:
\[\mathrm{v}^{\mathrm P}(\bs\kappa, \mb p_t) = \bar{\mathrm{u}} (\bs \kappa_t, \mb p_t) + \bar{\mathrm{e}} (\bs \kappa_t, \mb p_t) + \beta \mathrm V^{\mathrm{P}}(\bs\kappa_{t+1}), \]
and
\begin{equation}\label{eq:bellman_probability}
	\mathrm V^{\mathrm{P}}(\bs\kappa_t) = \max_{\mb p_t \in \mathcal{B}_P} \mathrm{v}^{\mathrm P}(\bs\kappa_t, \mb p_t) ,
\end{equation}
with $\bar{\mathrm{u}} (\bs \kappa_t, \mb p_t) = \bs\kappa_t\t \mb{u}( \mb{p}_t)$, $\bar{\mathrm{e}} (\bs \kappa_t, \mb p_t) = \bs\kappa_t\t \mb{e}( \mb{p}_t)$ and $\bs\kappa_{t+1} = \mb{F}( \mb{p}_t)\t \bs\kappa_t$.
% This is the \emph{dynamic probability-choice problem} associated with the original \emph{dynamic discrete choice model}.
The equation (\ref{eq:bellman_probability}) describes a reformulated Bellman equation of equation (\ref{eq:bellman}).
The following proposition establishes the equivalence between optimal decisions of the \emph{dynamic probability-choice problem} and the \emph{dynamic discrete choice model}. 
The proposition can be interpreted as, instead of choosing a discrete choice $d$ after the realizations of the state variables $(x,\epsilon)$, the agent chooses a complete plan $\mb p_t$ that maps the distributions of the state variables to a probability vector.


	\begin{lemma}\label{lemma:optimization_duality}
		Under assumption \ref{assumption:conditional_independence} to \ref{assumption:additive_seperable}, for a vector of the leave-one-out probability $\mb{p}(x) = [p(1,x),\ldots,p(D,x)]\t$,
		% and associated probability vector $\mb{\bar p}(x) = [p(0,x),\ldots,p(D,x)]\t$, 
		an arbitrary vector of continuation values $\mb{ v}(x) = [ v(0,x),\ldots, v(D,x)]\t$ and a vector of the expected private information variable $\mb e^{\mb p(x)}(x) = [e^{\mb p(x)}(0,x),\ldots,e^{\mb p(x)}(D,x) ]\t$ as defined in \eqref{eq:e_definition}. 
		Let \[ \mathrm{W}(\mb p(x), \mb v(x) ) = [1 - \iota\t \mb p(x), \mb p(x)\t] \left( \mb v(x) + \mb e^{\mb p(x)}(x) \right), \] where $\iota = [1,\ldots, 1]\t$.
		When $\mb p(x) = \bs \Lambda (\mb v (x))$, where $\bs{\Lambda}$ is the OCP mapping as defined in \eqref{eq:ocp_mapping}, we have 
		\begin{enumerate}
			\item 
			$\tilde v(d,x) + \tilde e^{\mb p(x)}(d,x) +  \nabla \mb e^{\mb p(x)}(d,x) = 0 $,
			where $\tilde{e}^{\mb p(x)}(d,x)  = e^{\mb p(x)}(d,x) - e^{\mb p(x)}(0,x)$ and $\nabla \mb e^{\mb p(x)}(d,x) = \sum_{d' \in \mathcal{D}} p(d',x) \frac{\partial e^{\mb p(x)}(d',x)}{\partial p(d,x)}$.
			\item $\frac{\partial  }{\partial p(d, x)} \mathrm{W}(\mb p(x), \mb v(x) ) = \tilde{\mathrm v}(d,x) - \bs{\Lambda}^{-1}(d,\mb p(x)),$
			where $\tilde v(d,x) = v(d,x) - v(0,x)$. 
		\end{enumerate}  
		where $\mb{u}( \mb{p}_t)(x)$ is the $x$-th element of $\mb{u}( \mb{p}_t)$ as in \eqref{eq:u_p} and $\mb{F}( \mb{p}_t) (x)$ is the $x$-th row of $\mb{F}( \mb{p}_t)$ as in \eqref{eq:F_p}. 
\end{lemma}
	
% Show the equivalence 
\begin{proposition}\label{prop:optimality}
	For any dynamic discrete choice problem and associated dynamic probability choice problem that satisfies Assumption \ref{assumption:conditional_independence} - \ref{assumption:additive_seperable}, and that $\kappa_t(x) > 0$ for all possible states $x\in\mathcal{X}$, the optimal probability choice of the Bellman equation (\ref{eq:bellman_probability}) is equal to the implied optimal choice probabilities from the solution to the discrete-decision Bellman equation (\ref{eq:bellman}).
\end{proposition}

	\begin{proof}[Proof of Proposition \ref{prop:optimality}] 
		We define an inter-temporal payoff function as $\mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t) = \bar{\mathrm{u}} (\bs \kappa_t, \tilde{\mb p}_t) + \bar{\mathrm{e}} (\bs \kappa_t, \tilde{\mb p}_t) + \beta \mathrm V^{\mathrm{P}}(\bs\kappa_{t+1})$, where we assume agent chooses an arbitrary probability(not necessarily optimal) $\tilde{\mb p}_t \in \mathcal{B}_P$ and choose optimally in subsequent periods. The agent receive expected payoffs $\bar{\mathrm{u}} (\bs \kappa_t, \tilde{\mb p}_t) + \bar{\mathrm{e}} (\bs \kappa_t, \tilde{\mb p}_t)$ at period $t$ and a discounted total value $\mathrm V^{\mathrm{P}}(\bs\kappa_{t+1})$ from $t+1$ onwards, with the transition $\bs \kappa_{t+1} = \mb{F}(\tilde{\mb p}_t ) \bs{\kappa}_t$.
		Rewrite $\mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t)$: 
		\begin{align*}
			\mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t) & = \bs{\kappa}_t\t \Big(\mb u(\tilde{\mb p}_t) + \mb e(\tilde{\mb p}_t) \Big) + \beta \mathrm{V}^{\mathrm{P}}(\bs \kappa_{t+1}), 
			% \\
			% & = \bs{\kappa}_t\t \Big(\mb u(\tilde{\mb p}_t) + \mb e(\tilde{\mb p}_t) \Big) + \beta \bs\kappa_{t+1}\t \Big(\mb u(\mb p_{t+1}) + \mb e(\mb p_{t+1}) + \beta \mathrm{V}^{\mathrm{P}}(\bs \kappa_{t+2}) \Big), \\
			% & = \bs{\kappa}_t\t \Big(\mb u(\tilde{\mb p}_t) + \mb e(\tilde{\mb p}_t)  + \beta  \mb{F}( \tilde{\mb p}_t)  \big(\mb u(\mb p_{t+1}) + \mb e(\mb p_{t+1}) + \beta \mathrm{V}^{\mathrm{P}}(\bs \kappa_{t+2}) \big) \Big).
		\end{align*}
		where $\mb u(\tilde{\mb p}_t)$, $\mb e(\tilde{\mb p}_t)$ and $\mb{F}( \tilde{\mb p}_t)$  are defined in \eqref{eq:u_p}, \eqref{eq:e_p} and \eqref{eq:F_p}.
		
		By Lemma \ref{lemma:optimization_duality}, for a public state and action pair $(d,x)$, the first order derivative is given by \begin{equation}
			\frac{\partial \mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t) }{\partial \tilde p(d,x)} = \kappa_t(x) \tilde u(d,x) + \beta \frac{\partial \mathrm{V}^{\mathrm{P}}(\bs \kappa_{t+1})}{\partial \bs \kappa_{t+1}} \frac{\partial \bs \kappa_{t+1}}{ \partial \tilde p(d,x) } - \kappa_t(x) \bs{\Lambda}^{-1}(d,\tilde{\mb p}_t(x)).
			\label{eq:partial_w_partial_p}
		\end{equation}
		
		We first show that $\partial \mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t)$ is globally concave in $\tilde{\mb p}_t$. Using the expression above to derive the first-order condition, and apply the inverse function theorem:
		\begin{equation*}\begin{split}
				\frac{\partial^2 \mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t) }{ \partial \tilde p(d,x) \partial \tilde p(d^{\dagger},x^{\dagger})} = \begin{cases} 0 & \text{ if } x \neq x^{\dagger} \\  
					- \kappa_t(x) \frac{\partial \bs{\Lambda}^{-1}(d,\tilde{\mb p}_t(x))}{\partial \tilde p(d^{\dagger}, x) } & \text{ if } x = x^{\dagger} . 
				\end{cases}
			\end{split}
		\end{equation*}
		Note that $\frac{\partial \bs{\Lambda}^{-1}(d,\tilde{\mb p}_t(x))}{\partial \tilde p(d^{\dagger}, x) } < 0$ if $d^{\dagger} \neq d$ and $\frac{\partial \bs{\Lambda}^{-1}(d,\tilde{\mb p}_t(x))}{\partial \tilde p(d^{\dagger}, x) } > 0$ if $d^{\dagger} = d.$
		% Magnus and Neudecker(1988) Theorem 29 establishes that this is equivalent to being positive definite.
		This implies that the Hessian matrix $\frac{\partial^2 \mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t) }{ \partial \tilde{\bs p} \partial \tilde{\bs p}\t}$ is negative definite and therefore $\mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t)$ is globally concave in $\tilde{\mb p}_t$.
		
		By the assumptions of the model, the inter-temporal payoff function is twice-continuously differentiable and globally concave in $\tilde{\mb p}_t$. Therefore the partial derivative $\partial \mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t) / \partial \tilde{\mb p}_t = 0$ characterize the unique optimal solution for $\mb p_t$. 
		Let $\mb p_{t+1}$, $\mb p_{t+2}, \ldots$ be the \eqref{eq:bellman} implied optimal choice probabilities for time $t+1$, $t+2$ and so on, then
		\begin{equation}
			\frac{\partial \mathrm{V}^{\mathrm{P}}(\bs \kappa_{t+1})}{\partial \bs \kappa_{t+1}\t} 
			% & = \mb u(\mb p_{t+1})\t + \mb e(\mb p_{t+1})\t + \beta \frac{\partial \mathrm{V}^{\mathrm{P}}(\bs \kappa_{t+2})}{\partial \bs \kappa_{t+2}} \frac{\partial \bs \kappa_{t+2}}{\partial \bs \kappa_{t+1}}, \\
			= \mb u(\mb p_{t+1}) + \mb e(\mb p_{t+1}) + \beta \bar{\mb F}(\mb p_{t+1}) \frac{\partial \mathrm{V}^{\mathrm{P}}(\bs \kappa_{t+2})}{\partial \bs \kappa_{t+2}\t} .
			\label{eq:partial_vp_partial_kappa}
		\end{equation}
		Note that $\frac{\partial \bs \kappa_{t+1}}{ \partial \tilde p(d,x) } = \kappa_t(x) \tilde{\mb f}(d,x)$, where  
		$\tilde{\mb f}(d,x) = [\tilde f(1|d,x),\ldots, \tilde f(X|d,x)]\t$ and $\tilde f(x'|d,x) = f(x'|d,x) - f(x'|0,x)$.
		By applying \eqref{eq:partial_vp_partial_kappa} recursively and plugging into \eqref{eq:partial_w_partial_p}, we have 
		\[\begin{split}
			\frac{\partial \mathrm{w}^{\mathrm P}(\bs\kappa_t, \tilde{\mb p}_t) }{\partial \tilde p(d,x)} & = \kappa_t(x) \tilde u(d,x)  - \kappa_t(x) \bs{\Lambda}^{-1}(d,\tilde{\mb p}_t(x)) + \\ & \kappa_t(x) \tilde{\mb f}(d,x)\t \Big( \sum_{s=1}^{T-t} \beta^s \Pi_{p=0}^{s-1} \bar{\mb F}(\mb p_{t+p}) \big(\mb u(\mb p_{t+1}) + \mb e(\mb p_{t+1}) 
			\big) \Big). 
		\end{split}\]
		The solution for the equation is given by $\mb p_t = \{  \mb p_t(x) = \bs{\Lambda}\left( \tilde{\mb w}(x) \right) : x \in \mathcal{X}\}$, and $\tilde{\mb w}(x) = \{ \tilde u(d,x) + \tilde{\mb f}(d,x)\t \Big( \sum_{s=1}^{T-t} \beta^s \Pi_{p=0}^{s-1} \bar{\mb F}(\mb p_{t+p}) \big(\mb u(\mb p_{t+1}) + \mb e(\mb p_{t+1}): d \in \mathcal{D} / \{ 0\} \}$.
		By definition, $\tilde{\mb w}(x) = \tilde{\mb v}(x)$ and by monotonicity of $\bs{\Lambda}$ the result follows.
	\end{proof}
	

 \begin{proof}[Proof of Lemma \ref{lemma:optimization_duality}]
		We write $\mathrm{W}(\mb p(x), \mb v(x))$ as 
		\begin{equation}\label{eq:value_function_probability_state_x}
			\mathrm{W}(\mb p(x), \mb v(x)) = \sum_{d \in \mathcal{D}} p(d,x)\left(\mb {\tilde v}(x) + {e}^{\mb p(x)}(d, x) \right) + v(0,x),
		\end{equation}
		% where $\mb{ \tilde v}(x) = [\tilde v(1, x), \ldots, \tilde v(D,x)]\t$ 
		% and $\mb {\tilde e}^{\mb p(x)}(x) = [\tilde e^{\mb p(x)}(1,x),\ldots, \tilde e^{\mb p(x)}(D,x)]\t$ with
		where $\tilde v(d,x) = v(d,x) - v(0,x)$.
		%  and $\tilde e^{\mb p(x)}(d,x) = e^{\mb p(x)}(d,x) - e^{\mb p(x)}(0,x).$
		When $\mb p(x) = \Lambda(\mb v(x))$.
		The total derivative of $\mathrm{W}(\Lambda(\mb v(x)), \mb v(x))$ with respect to $v(d,x)$ is 
		% \[\begin{split}
			%   \frac{d }{d \tilde v(d,x)}\mathrm{W}(\Lambda(\mb v(x)), \mb v(x)) = \sum_{d' \in \mathcal{D}} \frac{\partial }{\partial p(d',x)} \mathrm{W}(\Lambda(\mb v(x)), \mb v(x))  + \frac{\partial }{\partial v(d,x)} \mathrm{W}(\Lambda(\mb v(x)), \mb v(x)) 
			% \end{split}\]
		
		% We take the partial derivative of \eqref{eq:value_function_probability_state_x} with respect to $ \tilde v(d,x)$
		\[\begin{split}
			\frac{d}{d v(d,x)} & \mathrm{W}(\Lambda(\mb v(x)), \mb v(x)) \\ & = \frac{\partial }{\partial v(d,x)}  \mathrm{W}(\Lambda(\mb v(x)), \mb v(x))  + \sum_{d' \in \mathcal{D}} \left( \frac{\partial }{\partial p(d',x)} \mathrm{W}(\Lambda(\mb v(x)), \mb v(x)) \right) \left(\frac{\partial p(d',x)}{ \partial v(d,x)} \right).
			% \frac{\partial \Lambda(\mb v(x))(d,x)}{\partial v(d,x)}  (\tilde v(d,x) + \tilde e^{\mb p(x)}(d,x)) \\ & + \Lambda(\mb v(x))(d,x) (1 + \frac{\partial \tilde e^{\mb p(x)}(d,x)}{\partial p(d,x)} \frac{\partial \Lambda(\mb v(x))(d,x)}{\partial v(d,x)} ) - \frac{\partial e^{\mb p(x)}(0,x)}{\partial p(0,x)} \frac{\partial \Lambda(\mb v(x))(d,x)}{\partial v(d,x)} .
		\end{split}\]
		
		By the Williams-Daly-Zachery theorem, $\frac{\partial}{\partial v(d,x)} \mathrm{W}(\mb p(x), \mb v(x)) = p(d,x) $.
		By the definition of the optimal choice probability mapping, $\frac{\partial \Lambda(\mb v(x))(d,x)}{\partial v(d,x)} > 0$. 
		Then we have $\tilde v(d,x) + \tilde e^{\mb p(x)}(d,x) + \sum_{d' \in \mathcal{D}} p(d',x) \frac{\partial e^{\mb p(x)}(d',x)}{\partial p(d,x)} = 0$. 
		The second statement is shown by \cite{Aguirregabiria2016} Lemma 2.
		Note that $\mb{ \tilde v}(x) = \Lambda^{-1}(\mb p(x))$. Denote the $d$-th element as $\Lambda^{-1}(\mb p(x))(d,x)$. 
		We rewrite $\mathrm{W}(\mb p(x), \mb v(x))$ as $\mathrm{W}(\mb p(x), \Lambda^{-1}(\mb p(x)))$. 
	\end{proof}
	\begin{proof}[Proof of Lemma \ref{lemma:finite_dependence_variation}]
		If there exists such $\mb p_{t+1}^\dagger$ as stated, for any $\mb p_t, \mb p_t^* \in \mathcal{B}_P$, \\
		$\left(\mb{F}^{\mathrm P}(\mb p_t)\mb{F}^{\mathrm P}(\mb p_{t+1}^\dagger)\right) = \left(\mb{F}^{\mathrm P}(\mb p_t^*)\mb{F}^{\mathrm P}(\mb p_{t+1}^\dagger)\right)$. 
		If the model exhibits 1-period finite dependence, for any $(\mb p_t, \mb p_{t+1})$ there exists $(\mb p^*_t, \mb p^*_{t+1})$ such that $\mb{F}(\mb p_t) \mb{F}(\mb p_{t+1}) =  \mb{F}(\mb p^*_t) \mb{F}(\mb p^*_{t+1})$. 
		The above statement is equivalent to that for any $\mb p, \mb p_{t+1} \in \mathcal{B}_p$ there exists a pair of $(\mb p_t^*, \mb p_{t+1}^*) \neq (\mb p_t, \mb p_{t+1})$ such that
		\begin{equation}   
			\mb{F}(\mb p_t) \left(\mb{F}(\mb p_{t+1}) - \mb{F}(\mb p_{t+1}^\dagger) \right) = \mb{F}(\mb p_t^*) \left( \mb{F}(\mb p_{t+1}^*) - \mb{F}(\mb p_{t+1}^\dagger) \right). \end{equation}
		Let $\mb p_{t+1} = \mb p_{t+1}^*$. Note that the ranks of $\left( \mb{F}(\mb p_{t+1}^*) - \mb{F}(\mb p_{t+1}^\dagger) \right)$ and $\left( \mb{F}(\mb p_{t+1}^*) - \mb{F}(\mb p_{t+1})^\dagger \right)$ are not full.
		Therefore there exist non-unique values of $\mb p_t \neq \mb p_t^*$ such that the equation is satisfied.
	\end{proof}

 \begin{proof}[Proof of Proposition \ref{prop:two_period_finite_dependence}]
		We define the optimization problem of the agent in analogy to a continuous decision and continuous state problem. Let the agent problem be:
		
		$$
		\max_{\mathbf{p}_t, \mathbf{p}_{t+1}} \bar{u}(\boldsymbol{\kappa}_t, \mathbf{p}_t) + \bar{e}(\boldsymbol{\kappa}_t, \mathbf{p}_t) + \beta \left(\bar{u}(\boldsymbol{\kappa}_{t+1}, \mathbf{p}_{t+1}) + \bar{e}(\boldsymbol{\kappa}_{t+1}, \mathbf{p}_{t+1}) \right)
		$$
		
		subject to:
		
		$$
		\boldsymbol{\kappa}_{t+2} = \boldsymbol{\kappa}_{t} \mathbf{F}^{\mathrm{P}}(\mathbf{p}_{t}) \mathbf{F}^{\mathrm{P}}(\mathbf{p}_{t+1}).
		$$
		
		We show this characterization by demonstrating that the proposition holds for a 1-period finite dependent model. The result can then be easily extended to a $(\rho + 1)$-finite dependent model.
		The derivatives of the above optimization exploit the agent marginal trade-offs between the choice probabilities between the two consecutive periods. 
		We write the Lagrangian function of the constrained optimization as \begin{equation}\begin{split}
				\mathcal{L}(\mb p_t, \mb p_{t+1}, \bs{\tilde \lambda}) & = \bar u(\bs\kappa_t, \mb p_t) + \bar e(\bs\kappa_t, \mb p_t) + \beta \left( \bar u(\bs\kappa_{t}\mb F^{\mathrm P}(\mb p_t), \mb p_{t+1}) + \bar e(\bs\kappa_{t}\mb F^{\mathrm P}(\mb p_t), \mb p_{t+1}) \right) \\ & + \bs{\tilde \lambda}\t \Big(\bs \kappa_{t+2} - \mb F^{\mathrm P}(\mb p_{t+1})\t \mb F^{\mathrm P}(\mb p_{t})\t \bs \kappa_t \Big).
			\end{split}
		\end{equation}
		The Lagrangian function has multiple solutions only when the model exhibits the finite dependence property.
		Note that the derivative of $\mb u(\mb p_t)$, $\mb e(\mb p_t)$ and $\mb F(\mb p_t)$ as in \eqref{eq:u_p}, \eqref{eq:F_p} and \eqref{eq:u_p} with respect to $p_t(d,x)$ are $\tilde u(d,x) = u(d,x) - u(0, x)$, $\widetilde{\nabla e}^{\mb p_t(x)}(d,x) = \nabla e^{\mb p_t(x)}(d,x) - \nabla e^{\mb p_t(x)}(0,x) $ and $\tilde {\mb f}(d,x) = \mb f(d,x) - \mb f(0,x)$ for $d \in \mathcal{D} / \{ 0\}$ and $x \in \mathcal{X}$, where $\mb f(d,x) = [f(1|d,x), \ldots, f(X|d,x)]\t$ and $\nabla e^{\mb p_t(x)}(d,x) = \partial e^{\mb p_t(x)}(d,x)/ \partial p_t(d,x)$ for all $d \in \mathcal{D}$ and $x \in \mathcal{X}$, where $e^{\mb p_t(x)}$ is defined in \eqref{eq:e_definition}. 
		Let $\tilde \lambda (x^{\dagger\dagger})$ denote the $x^{\dagger\dagger}$-th element in the $\bs{\tilde \lambda}$ vector.
		Then first-order derivatives of the Lagrangian function with respect to $\mb p_t(d,x)$ and $\mb p_{t+1}(d^\dagger, x^\dagger)$ for $x, x^\dagger \in \mathcal{X}, d, d^\dagger \in \mathcal{D} / \{0 \}$ are
		\begin{equation}
			\begin{split}\label{eq:foc_xd_t}
				\frac{\partial}{\partial p_t(d,x)} \mathcal{L}(\mb p_t, \mb p_{t+1}, \bs{\tilde \lambda}) & = \kappa_t(x) \Big(\tilde u(d,x) + \tilde e_t^{\mb p(x)}(d,x) +  \nabla \mb e^{\mb p_t(x)}(d,x)  \Big)  \\ & + \beta \sum_{x^\dagger} \Big( \sum_{d^\dagger \in \mathcal{D}} p_{t+1}(d^\dagger,x^\dagger)  \big( u(d^\dagger, x^\dagger) + e^{\mb p_{t+1}(x^\dagger)}(d^\dagger, x^\dagger) \big) \Big) \tilde f(x^\dagger | d, x) \kappa_t(x) \\ & - \sum_{x^{\dagger \dagger}} \tilde\lambda(x^{\dagger \dagger}) \sum_{x^\dagger, d^\dagger} f(x^{\dagger \dagger}|d^\dagger, x^\dagger) p_{t+1}(d^\dagger, x^\dagger) \tilde f(x^\dagger | d, x) \kappa_t(x). 
			\end{split}
		\end{equation}
		and
		\begin{equation}
			\begin{split}\label{eq:foc_xd_t+1}
				\frac{\partial}{\partial p_t(d^\dagger,x^\dagger)} \mathcal{L}(\mb p_t, \mb p_{t+1}, \bs{\tilde \lambda})  & = \beta \sum_{x, d} \kappa_t(x) p_t(d,x) f(x^\dagger | d, x) \Big( \tilde u(d^\dagger, x^\dagger) + \tilde e_{t+1}^{\mb p(x^\dagger)}(d^\dagger, x^\dagger) \\ & +  \nabla \mb e^{\mb p_{t+1}(x^\dagger)}(d^\dagger, x^\dagger)   - \sum_{x^{\dagger\dagger}} \tilde\lambda(x^{\dagger\dagger}) \tilde f(x^{\dagger\dagger} | d^\dagger, x^\dagger) \Big),
			\end{split}
		\end{equation}
		where $\tilde{\mb F}(x)$ is a $D \times X$ matrix with $(d,x^\dagger)$-th element being $\tilde f(x^\dagger | d,x)$.
		With the assumption that $\kappa_t(x) \neq 0$,  stack the first order conditions with respect to $d \in \mathcal{D} / \{ 0 \}$ for any given $x$ in equation \eqref{eq:foc_xd_t} and we have 
		\[  \underbrace{\tilde{\mb u}(x)}_{D \times 1} + \underbrace{\tilde{\mb e}^{\mb p_t(x)}(x)}_{D \times 1} + \underbrace{\nabla \mb e^{\mb p_t(x)}(x)}_{D \times 1} +  \beta\underbrace{\tilde{\mb F}(x)}_{D \times X}  \left(  \underbrace{ \mb u(\mb p_{t+1}) + \mb e(\mb p_{t+1}) }_{X \times 1} \right)  -  \underbrace{\mb F(\mb p_{t+1})}_{X \times X} \underbrace{\bs\lambda}_{X \times 1}  = \mb 0. \]
		This proof is similar to that of \cite{arcidiacono2011conditional} and \cite{Aguirregabiria2016} if we assume $\kappa_t(x) = 1$ for some state $x \in \mathcal{X}$ and $0$ elsewhere. 
		Also we stack the first order conditions with respect to $d^\dagger \in \mathcal{D} / \{ 0 \}$ for any given $x^\dagger$ in equation \eqref{eq:foc_xd_t+1}  and have 
		\[ \beta  \left( \underbrace{\tilde{\mb u}(x^\dagger)}_{D \times 1} + \underbrace{\tilde{\mb e}^{\mb p_{t+1}(x^\dagger)}(x^\dagger)}_{D \times 1} + \underbrace{\nabla {\mb e}^{\mb p_{t+1}(x^\dagger)}(x^\dagger)}_{D \times 1} \right) - \underbrace{\tilde{\mb F}(x^\dagger)}_{D \times X} \underbrace{\bs\lambda}_{X \times 1} = 0. \]
		We let $u^{\mb p_{t+1}(x^\dagger)}(x^\dagger)$ and $e^{\mb p_{t+1}(x^\dagger)}(x^\dagger)$ be the $x^\dagger$-th elements of $\mb u(\mb p_{t+1})$ and $\mb e(\mb p_{t+1})$ and let $\mb f^{\mb p_{t+1}(x^\dagger)}(x^\dagger)$ be the $x^\dagger$-th row of $\mb F(\mb p_{t+1})$. 
		Note that $u^{\mb p_{t+1}(x^\dagger)}(x^\dagger) + e^{\mb p_{t+1}(x^\dagger)}(x^\dagger) = \left(\mb p_{t+1}(x^\dagger)\right)\t \left( \tilde{\mb u}(x^\dagger) + \tilde{\mb e}^{\mb p_{t+1}(x^\dagger)}(x^\dagger) \right) + u(0, x^\dagger) + e^{\mb p_{t+1}(x^\dagger)}(0,x^\dagger)$. 
		Also $\mb f^{\mb p_{t+1}(x^\dagger)}(x^\dagger) = \left(\mb p_{t+1}(x^\dagger)\right)\t \mb{\tilde F}(x^\dagger) + \mb f(0, x^\dagger)$, with $\mb f(0, x^\dagger)$ being the row vector of $f(x^\dagger | 0, x)$ for $x^\dagger \in \mathcal{X}$.
		For any weight vectors that satisfy the condition $\mb w_{t+1} \equiv \{ w(d^\dagger, x^\dagger): d \in \mathcal{D} / \{ 0\}, x \in \mathcal{X}\} \in \mathcal{B}_w$ such that $\sum_{d^\dagger \in \mathcal{D}} w(d^\dagger, x^\dagger) =1, ~ \forall x^\dagger \in \mathcal{X}$,
		we have 
		\[ \tilde{\mb u}(x) + \tilde{\mb e}^{\mb p_{t+1}(x)}(x) + \nabla \mb e^{\mb p_t(x)}(x) + \beta \underbrace{\tilde{\mb F}(x)}_{D \times X} \underbrace{\left( \mb u(\mb w_{t+1}) + \mb e^{\mb p_{t+1}}(\mb w_{t+1}) \right)}_{X \times 1} - \underbrace{ \tilde{\mb F}(x)}_{D \times X} \underbrace{\mb F(\mb w_{t+1})}_{X \times X} \underbrace{\bs\lambda}_{X \times 1}  = 0, \]
		where the $x^\dagger$-th elements of $\mb u(\mb w_{t+1})$ and $\mb e^{\mathbf p_t}(\mb w_{t+1})$ are $\mb w_{t+1}(x^\dagger)\t \tilde{\mb u}(x^\dagger) + u(0, x^\dagger)$ and 
		$\mb w_{t+1}(x^\dagger)\t ( \mb{\tilde e}^{\mb p_{t+1}(x^\dagger)}(x^\dagger) + \nabla{\mb e}^{\mb p_{t+1}(x^\dagger)}(x^\dagger) ) - \mb p_{t+1}(x^\dagger)\t \nabla{\mb e}^{\mb p_{t+1}(x^\dagger)}(x^\dagger) + e^{\mb p_{t+1}(x^\dagger)}(0, x^\dagger)$, respectively with $\mb w_{t+1}(x^\dagger)$ being the weight vector.
		If there exists a weight vector $\mb w_{t+1} \in \mathcal{B}_w$ such that $ \tilde{\mb F}(x)  \mb F(\mb w_{t+1}) = \mb 0$ for all $x \in \mathcal{X}$, then the optimal decision rule is characterized by 
		\[ \tilde{\mb u}(x) + \tilde{\mb e}^{\mb p_t(x)}(x) + \nabla \mb e^{\mb p_t(x)}(x) + \beta \underbrace{\tilde{\mb F}(x)}_{D \times X} \underbrace{\left( \mb u(\mb w_{t+1}) + \mb e^{\mb p_{t+1}}(\mb w_{t+1}) \right)}_{X \times 1} = \mb 0\] for all $x \in \mathcal{X}$. 
		Therefore, the model exhibits 1-period finite dependence.
	\end{proof}

==> sections/B2_lagrangian.tex <==
In a stationary model, the concept of finite dependence for a period $\rho + 1$ can be iterated in the following problem. Given any current state $x_t$, if we can identify a sequence of contingent actions based on the action performed $d_t$, the conditional distribution of the state in period $t + \rho$ remains invariant. It is crucial to note that this argument can be extended to non-stationary models as well.

We empower the agent to make conditional choices based on both a lagged state and the current state. In other words, for the conditional choice probability $p_{t+s}(x_{t+s}|x_{t+s-1})$, the agent's decision is influenced by both the past state ($x_{t+s-1}$) and the current state ($x_{t+s}$). It's noteworthy that under optimality, the conditional choice probability satisfies $\kappa_{t+s}(x_{t+\rho}|x_{t}) = \kappa_{t+\rho}^*(x_{t+\rho})$.

Shifting our focus to the Lagrangian maximization problem, let us represent the current state at time $t$ with the variable $x_t \in \mathcal{X}$, and denote the state at period $t+\rho+1$ by $j$.

The Lagrangian problem for the state $i$ that is realized at time $t$ is written as \[ \mathcal{L}(x_t) = \mathcal{U}(x_t) + (\mathcal{F}_t^{\rho}(x_t) - \mathcal{F}_t^{\rho,*}(x_t) ) \lambda.\]
We let the sum of flow utility from period $t$ across $t+\rho$  be represented by $\mathcal{U}(x_t)$, and we let the constraint be denoted using $\mathcal{F}_t^{\rho}(x_t)$, and $\lambda$ be the Lagrangian multiplier. 
Note that $\mathcal{F}_t^{\rho}(x_t)$ is the $i$-th row of $\mathcal{F}_t^{\rho}$.

The $(x_{t}x_{t+3})$-th element of $\mathcal{F}_t^{\rho}$ is written as 
\[ [\mathcal{F}_t^{\rho}]_{x_{t}, x_{t+3}} = \sum_{x_{t+1}} \sum_{x_{t+2}} \cdots \sum_{x_{t+\rho }} f^{\mathrm{e}}(x_{t+1}|x_t)  f^{\mathrm{e}}(x_{t+2}|x_{t+1}, x_t) \cdot  \ldots  f^{\mathrm{e}}(x_{t+\rho+1}|x_{t+\rho}, x_{t}) \]
where \[  
  f^{\mathrm{e}}(x_{t+s+1}|x_{t+s},x_{t+s-1}) = 
  \tilde{f}(x_{t+s+1}|x_{t+s}) p_{t+s}(x_{t+s}|x_{t}) + f_0(x_{t+s+1}|x_{t+s}), \]

We take the derivative with repsect to $p_t(x_t)$, and $p_{t+s}(x_{t+s}|x_{t})$.

Note that the objective function is written as 
\[\begin{split}  
  \mathcal{U}(x_t)  = u^{\mathrm{e}}(x_t) & + \beta \sum_{x_{t+1}} f^{\mathrm{e}}(x_{t+1} | x_t) \Big( p_{t+1}(x_{t+1}, x_t) \tilde{u}(x_{t+1}) + u_0(x_{t+1})  \Big) \\ 
& + \beta^2 \sum_{x_{t+1}} \sum_{x_{t+2}} f^{\mathrm{e}}(x_{t+1} | x_t) f^{\mathrm{e}}(x_{t+2} | x_{t+1}, x_t) \Big( p_{t+2}(x_{t+2}, x_{t}) \tilde{u}(x_{t+2}) + u_0(x_{t+2}) \Big). 
\end{split}
\]

Then the derivative of $\mathcal{L}(x_t)$ with respect to $p_{t+1}(x_{t+1}|x_{t})$ and $p_{t+2}(x_{t+2}|x_{t+1})$.
\begin{align}
 \partial \mathcal{L}(x_t) / \partial p_{t}(x_{t}) & = \tilde{u}(x_t) + \tilde{f}(x_{t+1 | x_t}) \Big( \beta \mathbf{u}^{\mathrm{e}}(x_{t+1}) \\
    & + \beta^2 \sum_{x_{t+2}}  f^e(x_{t+2} | x_{t+1}, x_t)    p_{t+2}(x_{t+2},x_{t}) \tilde{u}(x_{t+2}) + u_0(x_{t+2}) \Big\} 
    \nonumber \\
    & \left. + \sum_{x_{t+2}} f^e(x_{t+2} | x_{t+1}, x_t) \sum_{x_{t+3}} \left( f^{\mathrm{e}}(x_{t+3} |x_{t+2}, x_{t}) \lambda(x_{t+3}) \right) \right) = 0
  \label{eq:foc_t}
  \tag{t} \\
 \partial \mathcal{L}(x_t) / \partial p_{t+1}(x_{t+1}|x_{t}) & = f^{\mathrm{e}}(x_{t+1}|x_t) \Big(  \beta \tilde{u}(x_{t+1}) + \nonumber \\
    & \beta^2 \sum_{x_{t+2}} \tilde{f}(x_{t+2}|x_{t}) \left\{ p_{t+2}(x_{t+2},x_{t}) \tilde{u}(x_{t+2}) + u_0(x_{t+2}) \right\} \nonumber \\
    & + \sum_{x_{t+2}} \tilde{f}(x_{t+2}|x_{t+1}) \sum_{x_{t+3}} \left( f^{\mathrm{e}}(x_{t+3} |x_{t+2}, x_{t}) \lambda(x_{t+3}) \right) \Big) = 0   \label{eq:foc_t+1}  \tag{t+1} \\
\partial \mathcal{L}(x_t) / \partial p_{t+2}(x_{t+2}|x_{t}) & = f^{\mathrm{e}}(x_{t+1}|x_t) f^{\mathrm{e}}(x_{t+2}|x_{t+1},x_{t}) \nonumber\\
    &\quad \Big( \beta^2 \tilde{u}(x_{t+2}) + \sum_{x_{t+3}} \left( \tilde{ f}(x_{t+3} | x_{t+2}) \lambda(x_{t+3}) \right) \Big) = 0
  \label{eq:foc_t+2} \tag{t+2}
\end{align}

From \eqref{eq:foc_t+2}, we get 
\begin{equation}
  \beta^2 \tilde{u}(x_{t+2}) + \sum_{x_{t+3}} \left( \tilde{ f}(x_{t+3} |x_{t+2}) \lambda(x_{t+3}) \right) = 0. \label{eq:foc_t+2'}
  \tag{t+2'}
\end{equation}
Plug in back to get 

\begin{equation}
  \begin{aligned}
    \beta\tilde{u}(x_{t+1}) & + \beta^2 \sum_{x_{t+2}} \tilde{f}(x_{t+2}|x_{t+1})  \left\{ w_{t+2}(x_{t+2},x_{t+1}) \tilde{u}(x_{t+2}) + u_0(x_{t+2}) \right\} \\
    & + \sum_{x_{t+2}} \tilde{f}(x_{t+2}|x_{t+1}) \sum_{x_{t+3}} \left( w_{t+2}(x_{t+2},x_{t}) \tilde{f}(j | x_{t+2}) + f_0(x_{t+3} | x_{t+2}) \right) \lambda(x_{t+3}) = 0,
  \end{aligned}
  \label{eq:foc_t+1'}
  \tag{t+1'}
\end{equation}
where the weight $w_{t+2}(x_{t+2},x_{t}) \in \R$ is an real number that does not need to between 0 and 1.


==> sections/B3_matrix_representation.tex <==

\section{Linear Estimator}

We write the expression of $\tilde{v}(x_t, d_t)$ as a function $\mathbf{\check w}_{x}$:
\[
\begin{split}
\tilde{v}(x_t, d_t)  = \tilde{u}(x_t, d_t) & + \beta \sum_{x_{t+1}}  \mathrm{\check w}_{(x_t, d_t)}(d_{t+1},x_{t+1}) \Big( \tilde{u}(d_{t+1},x_{t+1}) + \tilde{e}(d_{t+1},x_{t+1})  + \beta \tilde{\mathbf f}(d_{t+1},x_{t+1}) \mathbf{V}_{t+1}\Big)  \\
& + \beta \sum_{x_{t+1}}  \tilde{f}(x_{t+1} | x, d ) \left( u(0,x_{t+1}) + e(x_{t+1}, 0) + \beta \mathbf f (0,x_{t+1}) \mathbf{V}_{t+1} \right).
\end{split}
\]
Re-organize the notations and get 
\[ 
\begin{split}
\tilde{v}(x_t, d_t)  &= \underbrace{ \tilde{u}(x_t, d_t)  + \beta \Big( \sum_{x_{t+1}}  \mathrm{\check w}_{(x_t, d_t)}(d_{t+1},x_{t+1}) \tilde{u}(d_{t+1},x_{t+1}) + \sum_{x_{t+1}}  \tilde{f}(x_{t+1} | x, d ) u(0,x_{t+1}) \Big) }_{\mathbf{H}(x,d, \mathbf{w}_{(x_t, d_t)})^\top \theta: \text{ Linear function of $\theta$. }}
\\ & 
+ \beta \underbrace{\Big( \sum_{x_{t+1}}  \mathrm{\check w}_{(x_t, d_t)}(d_{t+1},x_{t+1}) \tilde{e}(d_{t+1},x_{t+1}) + \sum_{x_{t+1}}  \tilde{f}(x_{t+1} | x, d ) e(0,x_{t+1}) \Big)}_{ \mathbf{h}(x,d, \mathbf{w}_{(x_t, d_t)}, \mathbf{\hat P}): \text{ Function of $p$, updated in each iteration}}
\\ &
+ \beta^2 \underbrace{\Big(  \sum_{x_{t+1}}  \mathrm{\check w}_{(x_t, d_t)}(d_{t+1},x_{t+1}) \tilde{\mathbf f}(d_{t+1},x_{t+1}) + \sum_{x_{t+1}}  \tilde{f}(x_{t+1} | x, d )  \mathbf f (0,x_{t+1})  \Big)}_{ \tilde{\mathbf{F}} \mathbf{F}(\mathbf{w}): \text{Bias correction mapping, can be computed before entering iterative methods}} \mathbf{V}_{t+1}  
\end{split}
\]

With $\rho$-period, the the value difference vector $\mathbf{\tilde v} \equiv\{ \tilde v(x_t, d_t) ,~ x \in \mathcal{X}, d \in \mathcal{D}\}$ at the current period is expressed as 
\[
\begin{split}
    \mathbf{\tilde v} & = \underbrace{\mathbf{\tilde u} + \sum_{s=1}^{\rho} \beta^s \big(  \mathbf{\check w}_{t+s} \mathbf{\tilde u} + \mathbf{\tilde F} \mathbf{F}(\mathbf{w}_{t+1}) \ldots \mathbf{F}(\mathbf{w}^{(s-1)}) \mathbf{u}_0 \big))}_{ \text{Linear in $\theta$ }, \mathbf{H}(x,d, \mathbf{w}_{t+1}, \ldots, \mathbf{w}_{t+\rho} )^\top \theta  } \\ 
    & + 
    \underbrace{ \sum_{s=1}^{\rho} \beta^s \big(  \mathbf{\check w}_{t+s} \mathbf{\tilde e}(\mathbf{P}) + \mathbf{\tilde F} \mathbf{F}(\mathbf{w}_{t+1}) \ldots \mathbf{F}(\mathbf{w}^{(s-1)}) \mathbf{e}_0(\mathbf{P}) \big)}_{\mathbf{h}(x,d, \mathbf{w}_{t+1}, \ldots, \mathbf{w}_{t+\rho}, \mathbf{\hat P}) } \\
	&  + \underbrace{
    \beta^{(\rho+1)} \big( \mathbf{\check w} \mathbf{\tilde F} + \mathbf{\tilde F} \mathbf{F}(\mathbf{w}_{t+1}) \ldots \mathbf{F}(\mathbf{w}_{t+\rho-1}\mathbf{F}_0\big)}_{\text{Bias correction mapping} = 0 } \mathbf{V}
\end{split}
\]
